On Higher Representation Theory via Categories of type Charge-Conserving--with--Glue

In this paper we introduce a strict monoidal subcategory of the category of matrices, suitable to address a higher representation theoretic analogue of radicals (non-semisimplicity) in ordinary representation theory. We show the extent to which this analogue has analogous representation theoretic properties. To illustrate, we apply to two key problems in the study of braid representations (strict monoidal functors from the braid category $\mathsf{B}$ to the matrix category): the classification problem; and the problem of analysing the ordinary braid group representations that braid representations generate in towers.

==> tex/macros-thesis.tex <==
\usepackage[all,knot]{xy}
\usepackage{graphicx} % Required for inserting images
\usepackage[utf8]{inputenc}
\usepackage[utf8]{inputenc}
\usepackage{amsmath}
\usepackage{bbm}    %% for \mathbbm ?
\usepackage{amssymb}
\usepackage{mathtools}
\usepackage{enumerate}
\usepackage{xcolor} 
\usepackage{amsthm} 
\usepackage{tikz}   
\usepackage{graphicx}
\usepackage{tikz-cd}
\usepackage{url}
\usepackage{ytableau}
\usepackage{hyperref} %% ppm: I think this makes refs into links.
\usepackage[normalem]{ulem} %% ppm: for striking out old text.
\theoremstyle{definition}
\newcommand{\Symm}[1]{\Sigma_{#1}}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}{Corollary}[theorem]
\newtheorem{remark}[theorem]{Remark}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{Remark}[theorem]{Remark}
 \newtheorem{example}[theorem]{Example}
\newtheorem{exercise}[theorem]{Exercise}
\usepackage{amsmath} 
\newcommand\inner[2]{\langle #1, #2 \rangle}
\newcommand{\tens}%[1]{\mathbin{\mathop{\otimes}\limits_{#1}}%
{\otimes 
}

\newcommand{\cc}{charge-conserving}   %%choose to hyphentate %% 
\newcommand{\acc}{additive \cc}
\newcommand{\ignore}[1]{}
\newcommand{\sss}[1]{\subsection{#1}}

\usepackage{ulem}
\usepackage{todonotes}
\usepackage[all]{xy}


%%% Macros transferd from the macros file.

\newcommand{\SET}{{\mathbf Set}}
\newcommand{\GRP}{{\mathbf Grp}}
\newcommand{\MATCH}{\mathbf Match}
\newcommand{\MAT}{{\mathbf Mat}} 
\newcommand{\VEC}{\mathbf Vec}

\newcommand{\ssa}[1]{\textcolor{blue}{#1}}
\newcommand{\aaa}[1]{\textcolor{purple}{#1}}
\newcommand{\MATCHA}{\MAT_{ACC}}
\newcommand{\botimes}{ \bar{\tens} }
\newcommand{\ssss}[1]{#1} % Define \ssss subsectios
\newcommand{\ppmadd}[1]{\textcolor{brown}{#1}}
\newcommand{\ppm}[1]{\textcolor{red}{#1}}
%\newcommand{\ppmx}[1]{}  
\newcommand{\kk}{{\mathbbm{k}}}
\newcommand{\C}{{\mathbb{C}}}  % here is our macro for complex field
\newcommand{\R}{{\mathbb{R}}}%here is our macro for real numbers
\newcommand{\N}{{\mathbb{N}}}  % here is our macro for natural numbers
\newcommand{\Z}{{\mathbb{Z}}}  % here is our macro for integer numbers
\newcommand{\Q}{{\mathbb{Q}}}  % here is our macro for rational field
\newcommand{\codt}{{\mathbf Dot product}} 
\newcommand{\beq}{\begin{equation}}
\newcommand{\eq}{\end{equation}}
\newcommand{\p}{P}  %% trying to fix your errors.
\newcommand{\ppmx}[1]{}  
\newcommand{\ppmm}[1]{#1}  
\newcommand{\Lamm}[2]{\Lambda^{#1}_{#2}}  % set of compositions 
\newcommand{\lamm}{{\bf m}}
\newcommand{\B}{{\mathbb{B}}}

%%%%this is macros-mdef
\newcounter{minidef}[section]
\renewcommand{\theminidef}{\thesection.\arabic{minidef}}
\newcommand{\mdef}{\refstepcounter{theorem}       \medskip \noindent ({\bf \thetheorem}) }
%\newcommand{\mdef}{\refstepcounter{thm}       \medskip \noindent ({\bf \thethm}) }

\newcounter{minicapt}
\newenvironment{capt}[1]
{\refstepcounter{minicapt}\stepcounter{figure}
\begin{center}\sf Figure \theminicapt. }{ \end{center}}

\newcommand{\PP}{{\mathsf{P}}}
\newcommand{\Bcat}{{\mathsf B}}  %% cat of braids

%\usepackage{tkz-euclide}
\usepackage{pst-plot}
\usetikzlibrary{positioning}
\usepackage{pgfplots}
\usepackage{pifont}
\pgfplotsset{compat = newest}
\usepackage{pictexwd,dcpic}

\newcommand\myeq{\mathrel{\overset{\makebox[0pt]{\mbox{\normalfont\tiny\sffamily Mult A,B}}}{=}}}
\newcommand\mmyeq{\mathrel{\overset{\makebox[0pt]{\mbox{\normalfont\tiny\sffamily Mult A,B,C}}}{=}}}
\newcommand\mmmyeq{\mathrel{\overset{\makebox[0pt]{\mbox{\normalfont\tiny\sffamily Mult assoc}}}{=}}}
\newcommand\mmmmyeq{\mathrel{\overset{\makebox[0pt]{\mbox{\normalfont\tiny\sffamily ret comp}}}{=}}}

